CRACKS: Crowdsourcing Resources for Analysis and Categorization of Key Subsurface faults

Crowdsourcing annotations has created a paradigm shift in the availability of labeled data for machine learning. Availability of large datasets has accelerated progress in common knowledge applications involving visual and language data. However, specialized applications that require expert labels lag in data availability. One such application is fault segmentation in subsurface imaging. Detecting, tracking, and analyzing faults has broad societal implications in predicting fluid flows, earthquakes, and storing excess atmospheric CO$_2$. However, delineating faults with current practices is a labor-intensive activity that requires precise analysis of subsurface imaging data by geophysicists. In this paper, we propose the $\texttt{CRACKS}$ dataset to detect and segment faults in subsurface images by utilizing crowdsourced resources. We leverage Amazon Mechanical Turk to obtain fault delineations from sections of the Netherlands North Sea subsurface images from (i) $26$ novices who have no exposure to subsurface data and were shown a video describing and labeling faults, (ii) $8$ practitioners who have previously interacted and worked on subsurface data, (iii) one geophysicist to label $7636$ faults in the region. Note that all novices, practitioners, and the expert segment faults on the same subsurface volume with disagreements between and among the novices and practitioners. Additionally, each fault annotation is equipped with the confidence level of the annotator. The paper provides benchmarks on detecting and segmenting the expert labels, given the novice and practitioner labels. Additional details along with the dataset links and codes are available at $\href{https://alregib.ece.gatech.edu/cracks-crowdsourcing-resources-for-analysis-and-categorization-of-key-subsurface-faults/}{link}$.

==> Sections/1_Introduction.tex <==
\section{Introduction}
\label{sec:Intro}
Understanding Earth’s subsurface structures via seismic image analysis has been and continues to be an essential component of various applications such as earthquake monitoring, carbon sequestration, and hydrocarbon exploration. Typically, geophysical expert interpreters first assume a geological model based on the analysis of various attributes of seismic data, in addition to the geological history of the region~\cite{alregib2018subsurface}. Thereafter, interpreters segment various subsurface structures of interest. An important subsurface structure that has broad societal impact is faults. Fig.~\ref{fig:Concept} illustrates the process used by an expert interpreter to segment a fault in the earth's subsurface. A fault is defined as a lineament or planar surface across which apparent relative displacement occurs in the rock layers. Visually, the fault is apparent, even to non-geophysicists, as discontinuities in the earth's subsurface. Geophysicists model the dominant structures (colored regions on the left image in Fig.~\ref{fig:Concept}) and check for discontinuities. However, non-geophysicists fall short when segmenting faults in the following cases: (i) it is not always clear where a fault starts and where it ends, and (ii) it is not always clear when there are a series of minor faults or there is one major fault. For instance, consider the cyan segmented region in Fig.~\ref{fig:Concept} as our region of interest (ROI). While the region above and below (in purple) the ROI shows displacement, there is no displacement within the ROI itself. Additionally, the magnitude of displacement within the yellow and red regions below the ROI is much larger than the purple region above the ROI. This indicates two separate faults. Further, the red and yellow regions to the left of the fault are next to each other while they deviate to the right of the fault. This indicates a series of minor faults. Note that this analysis requires geological study and structural segmentation from expert geophysicists.

\begin{figure}[t]
\centering
\includegraphics[scale =.5]{neurips_data_2023/Figs/Expert_Interpretation.png}
\vspace{-1.5mm}
\caption{Expert interpretation of a seismic fault.}\label{fig:Concept}\vspace{-3mm}
\end{figure}

\textbf{Societal impact} Analyzing and monitoring faults has multifarious societal benefits. Faults may be sources of societal hazard that allow earthquakes, sometimes exacerbated by human activities. Faults in the subsurface can serve as conduits to fluid-flow. Decades of experience has proven that CO$_2$ can be stored and sealed within the earth's subsurface, provided that there are no leakage pathways generated through reactivation of faults. This is termed carbon sequestration and it allows capturing and storing excess atmospheric carbon dioxide with the goal of reducing global climate change~\cite{warwicknational}. However, carbon dioxide may leak back into the atmosphere if there are are unknown non-sealing faults in the injection sites, requiring fault delineation before sequestration.

\textbf{Automating fault delineation} Fault delineation is the combined process of detecting and segmenting faults. As illustrated in Fig.~\ref{fig:Concept}, fault delineation process is time consuming and labor intensive \cite{mustafa2024visual}. Automated and semi-automated interpretation through computational algorithms have been investigated~\cite{wang2016interactive, cohen2006detection, roberts2001curvature, di2017seismic, shafiq2018towards, kokilepersaud2022volumetric}. However, training generalizable machine learning algorithms require labeled fault datasets which is lacking. Seismic surveys have grown over the years in both complexity and data sizes. However, different subsurface regions within the earth have different geologies, all of which cannot be labeled by geophysicists. To tackle this challenging situation, a common practice is to utilize synthetic data to construct deep learning models~\cite{wu2019faultseg3d, li2022automatic, shafiq2018towards, shafiq2018leveraging}. Synthetic data offers the advantage that the exact segmentation of faults is available. However, this is not realistic. Real data suffers from confounding factors that have not yet been modeled synthetically. This is specifically true in faults, where factors like earthquake epicenter depths create significant uncertainties~\cite{vakarchuk2019effect}. 

\textbf{CRACKS Dataset Contributions} To alleviate the lack of expertise, we propose the \texttt{CRACKS} dataset, the first subsurface fault-labeled data utilizing resources from crowdsourcing platforms. Specifically, we provide annotations from multiple expertise levels, of differing confidence, including from novices, practitioners, and an expert. We show that the noisy annotations from novices and practitioners are not trivial and can be utilized to model expert annotations. Annotations from multiple novices on the same image have large disagreements between them and from the expert. This allows \texttt{CRACKS} dataset to be used in a non-traditional way where the same images used during training with novice and practitioner labels can be used during inference to model expert annotations. 

==> Sections/2_LitReview.tex <==
\section{Related Work}
\label{sec:LitReview}
\paragraph{Seismic Data} Seismic images are obtained via transmitting and receiving signals, generally acoustic waves, through the earth's subsurface across a predefined survey area. Seismic image characteristics are dependent on the subsurface geology. Subsurface under the Netherlands North Sea F3 block~\cite{F3_data} has its own unique characteristics, distinct from other regions like Great South Basin in New Zealand~\cite{carter1988post}, and the South China Sea~\cite{chen2011seismic}. In this paper, we annotate faults on the Netherlands F3 block due to the following reasons:

\begin{itemize}
    \item The F3 block, apart from faults, has other dominant structures in the subsurface images. This provides a larger diversity in image features for deep learning algorithms to learn from.
    \item The F3 block is available for use publicly with no additional licensing and has a number of other annotations including structural interpretations in LANDMASS~\cite{alaudah2018structure} and Facies~\cite{alaudah2019machine} annotations. These annotations are not fault related but can be used as pretext tasks~\cite{kokilepersaud2022volumetric}.
    \item The F3 block has been used for a number of machine learning applications including contrastive learning~\cite{kokilepersaud2022volumetric}, active learning~\cite{benkert2023samples, mustafa2021man}, visual explainability~\cite{prabhushankar2020contrastive, alregib2022explanatory}, and model~\cite{benkert2022reliable} and label uncertainty estimation~\cite{zhou2023perceptual} among others.
    \item The faults in F3 block are easier to visually inspect and label as compared to polygonal faults in other parts of the earth's subsurface~\cite{carter1988post, chen2011seismic}. This ensures that specialized seismic software like OpendTect~\cite{dgbpy_2019} is not required for crowdsourced labeling.
\end{itemize}

\paragraph{Leveraging Crowdsourcing for Learning Expert Labels} Crowdsourcing labels from multiple annotators has been a common approach to obtain large labeled data. Crowdsourcing has fostered ML research in common knowledge applications including image classification \cite{peterson2019human, collins2022eliciting} and natural language processing \cite{uma2021learning, poesio2019crowdsourced}. However, specialized applications that require domain expert annotations lag in label availability. Some medical applications involve collecting annotations from multiple observers. However, the number of observers is typically small and the labeling is time-consuming \cite{armato2011lung, litjens2012pattern, almazroa2017agreement, menzequantification}. \texttt{CRACKS} is the first dataset that leverages crowdsourcing resources for delineating expert-labeled faults from annotators with limited and no expertise. For comparison, we summarize various key characteristics of the datasets that leverage crowdsourcing or provide multiple annotations in Table~\ref{tab:stats_datasets}. Note that none of these datasets are specifically for seismic data. Many of these datasets do not provide annotations from real expertise hierarchies. In certain specialized domains such as the medical domain, gold labels are usually derived from the majority voting among a few observers. However, majority voting rarely produces ground truth-expert labels in fault delineations due to various levels of labeling consistency and disagreement across different expertise levels. Even in medical data, arbitration between stakeholders is required~\cite{prabhushankar2022olives}. Compared to other datasets, \texttt{CRACKS} provides real-world settings where crowdsourcing from multiple levels of expertise can be used as an alternative to time-consuming labeling by experts. This unique characteristic of \texttt{CRACKS} facilitates the development of fine-tuning strategies that use limited expert labels to fine-tune ML models trained using a large number of labels from less experienced annotators, such as practitioners and novices. The availability of crowdsourced labels from different expertise levels also encourages benchmarking of self-supervised learning \cite{chen2020simple}. In addition to multiple levels of expertise, \texttt{CRACKS} also provides three categories of annotation confidence, which can be used for weighted or fused labels during training to enhance generalizability. Finally, \texttt{CRACKS} provides multiple tasks of interest including detection and instance segmentation \cite{glenn_jocher_2022_7347926}. To the best of our knowledge, \texttt{CRACKS} is the first subsurface fault dataset that provides crowdsourcing annotations from multiple levels of expertise with three types of labeling confidence.  

% Existing techniques can be categorized into two branch attempts to train models on data associated with a group of annotations collected from multiple practitioners or novices who have limited experience in labeling. The objective of the methods in this line of work is to fit a model predicting a set of labels that mimics the patterns of manual label disagreement. For example, Kohl et al. \cite{kohl2018probabilistic} proposed to model various label patterns for the segmentation task using a variational autoencoder. PHiSeg \cite{baumgartner2019phiseg} models segmentation label variability at different resolutions using hierarchical latent variables with sophisticated probabilistic architectures. Supervised Uncertainty Quantification (SupUQ) \cite{hu2019supervised} further estimates calibrated label disagreements by using inter-annotator variation as a means of supervision. \cite{kohl2018probabilistic, hu2019supervised} both can generate multiple modes of labeling hypotheses. These methods assume that multiple labels are collected from labelers at the same expertise level. However, they are less effective in estimating expertise-based label disagreement because they calculate label variation with respect to the mean of all practitioner labels, which is largely different from expert ground truths, especially in domains such as fault interpretation. Another line of modeling methods \cite{zhang2023learning, liao2024modeling} attempts to learn annotator-specific labeling patterns that are different from expert gold labels. These methods devise designated modules for imperfect annotators such as practitioners. Zhang et al. \cite{zhang2023learning} proposed to predict spatial error characteristics of individual annotators. Specifically, they assume that there exist unique pixel-wise class confusion matrices between an expert and each annotator. However, in the fault segmentation application, the probabilistic class transition from expert labels to practitioner labels can be dominated by the prevalence of the class of no-faults due to label sparsity. Furthermore, they require a fixed number of annotators thereby not being scalable to characterize different manifestations of large groups.

% \subsection{Efficient Expertise-based Data Labeling}
% Many frameworks utilize different levels of labeling expertise to improve labeling quality or enhance model performance while reducing the number of expert annotations. Some methods attempt to improve the quality of crowd-sourced annotations. Khattak et al. \cite{khan2012improving} proposed a quality-controlled labeling scheme using a few expert-labeled samples to estimate the expertise of individual crowd labelers, which is used to approximate the true labels for all data. However, they used crowd labelers to annotate all data without considering the optimal labeling budget. Li et al. \cite{li2015cheaper} proposed to select a subgroup of labelers that achieves the highest labeling accuracy with a budget constraint by solving a combinatorial optimization problem. However, these methods do not study the impact of crowd labels on the performance of networks. Correia et al. \cite{correia2019hybrid} stressed the increasing requirement of developing systems in which domain experts, crowd labelers, and networks interact with each other to solve complex tasks. Yang et al. \cite{yang2019predicting} proposed a framework that predicts annotation difficulty and assigns difficult samples to domain experts to achieve better model performance. Similar to our disagreement definition, they define sample difficulty as the disagreement between the expert and lay annotators. However, their framework can not generate various patterns of annotations and observe label disagreement. Mendez et al. \cite{mendez2019machine} devised a bi-direction system where the forward machine-crowd-experts loop seeks to enhance annotation quality and model performance, and the backward machine-expert-crowd loop aims to increase annotator engagement. However, they select uncertain samples for crowd labelers to annotate based only on model representations, which do not estimate annotator label disagreement and can be less effective. These methods leverage crowd labelers directly or combine a large number of crowd labelers and a few experts in labeling tasks and optimize labeling costs. However, they either did not study the impact of combining lay annotators and experts on model performance, or did not model annotator label patterns and disagreements to provide informative guidance for expertise resource allocation. Our approach aims to address these limitations.

\input{neurips_data_2023/Tables/2_DatasetCompare}



==> Sections/3_Dataset.tex <==
\input{neurips_data_2023/Tables/1_Stats}
\begin{figure}[t]
\centering
\includegraphics[scale =.4]{neurips_data_2023/Figs/challenges.jpg}
\vspace{-1.5mm}
\caption{Expert/Practitioner/Novice annotation of seismic sections.}\label{fig:challenges}\vspace{-3mm}
\end{figure}
\vspace{-3mm}
\section{Dataset Details}
\label{sec:Dataset}
\vspace{-3mm}
Table~\ref{tab:stats_datasets} shows the statistics of \texttt{CRACKS} dataset. Each section from the F3 block is an image of resolution $255 \times 701$ pixels with $255$ pixels placed along the depth from the surface of the earth. There are $400$ such sections, with an average of $19$ faults in each section. More details regarding the geological model is available in Appendix~\ref{subsec:F3}. 
\vspace{-3mm}
\paragraph{Amazon Mechanical Turk Setup} We leverage the Amazon Mechanical Turk (MTurk) platform to crowdsource fault annotations, adapting existing image segmentation layouts to suit our needs. In particular, we divide the 400-section F3 dataset into 20 batches consisting of 20 Human Intelligence Tasks (HITs), each batch corresponding to a single section. The data collection process was deemed to be Minimal risk research qualified for IRB exemption status under 45 CFR 46 104d.2 (Protocol H23360). All annotators are between 18 – 89 years old, and are able to consent without requiring surrogate consent from a legally authorized representative. Screenshots from the MTurk setup as well as other details are provided in Appendix~\ref{subsec:MTurk_setup}.
\vspace{-3mm}
\paragraph{Annotation Expertise} Annotations in \texttt{CRACKS} dataset are sourced from 26 novices, 8 practitioners, and a geophysicist. The novices, practitioners and geophysicist label on the same seismic sections from the F3 block. Hence, there are $35$ annotations per fault (Table~\ref{tab:stats_datasets}, column 3). Our definition of expertise is as follows:\vspace{-3mm}
\begin{itemize}
    \item \textbf{Novices} Recruits from MTurk with no experience interacting with subsurface sections and faults. To guide the labeling task, the novices are shown a \href{https://www.youtube.com/watch?v=Fyr4b_RiT8s}{5 min instructional video} that introduces faults and fault annotation on the MTurk platform. More information regarding worker compensation, labeling instructions, and eligibility is present on our \href{https://alregib.ece.gatech.edu/fun-ml-fault-uncertainty-for-machine-learning/}{participation call webpage} as well as Appendix~\ref{sec:AppC}.
    \item \textbf{Practitioners} Practitioners are graduate students who have previously worked with seismic data. However, they have not specifically labeled faults. The same \href{https://alregib.ece.gatech.edu/fun-ml-fault-uncertainty-for-machine-learning/}{participation call webpage} applies to practitioners, except participation is limited to Georgia Tech students.
    \item \textbf{Expert} A geophysicist acted as the labeling expert. The sixth column in Table~\ref{tab:stats_datasets} with $7636$ samples in \texttt{CRACKS} refer to the number of faults annotated by the expert. 
\end{itemize}

\paragraph{Annotation Confidence Types} Four exemplar seismic sections along with randomly selected novice, practitioner, and the expert labels are shown in Fig.~\ref{fig:challenges}. The color of the labels (blue, green, or orange) depicts the confidence of the annotators for that fault. Confidence definitions are as follows:
\begin{itemize}
    \item \textbf{No fault (certain)}: This category is used to demarcate regions where the annotator is sure of the absence of any seismic faults. This region is annotated in orange in Fig.~\ref{fig:challenges}.
    \item\textbf{Fault (certain)}: Used to delineate seismic faults of whose existence the annotator feels fairly confident in. We use the color blue for this category in Fig.~\ref{fig:challenges}. 
    \item \textbf{Fault (uncertain)}: Used to delineate faults that are only partially discernible or are otherwise not fully ascertainable by the annotator. We use the color green for this category in Fig.~\ref{fig:challenges}. 
\end{itemize}
The specifics of the brush tool used to obtain these annotations on MTurk platform are provided in Appendix~\ref{subsec:MTurk_setup}. In Table~\ref{tab:stats_data}, we show the number of certain and uncertain faults labeled by the expert geophysicist and aggregates of all $26$ novices and $8$ practitioners. Interestingly, of the $7636$ faults labeled by the expert, only $815$ faults are certain. This is only $14.5\%$ of all faults labeled by the geophysicist. In contrast, $48.1\%$ of all faults labeled by the novices are certain. However, in accordance with our granted IRB exemption, we do not collect any behavioral data that may lead to analyzing this confidence inequity. Additionally, averaged percentage of pixels in each section describes the class-imbalance issues in section-wise segmentation.
\vspace{-3mm}
\paragraph{Annotation Quality Control} To ensure quality of obtained labels, each batch of $20$ HITs is augmented twice with 2 redundant and randomly selected seismic sections from the batch. Hence, every batch has $24$ sections, out of which only $20$ are unique. None of the annotators across expertise are told this in order to perform a quality assurance (QA) analysis. Hence, we obtain $120$ quality assessment (QA) sections ($40$ sections repeated thrice) within the dataset to evaluate annotator self-consistency. We use three metrics - modified Hausdorff distance, mean Intersection over Union (mIOU), and DICE coefficient to measure this self-consistency. The specifics of the metrics are presented in Appendix~\ref{subsec:Metrics}. Hausdorff distance is sensitive to the boundary of the faults while mIOU and DICE coefficients are sensitive to the areas of the fault. All three metrics are commonly used to quantify fault delineation~\cite{dou2021attention} as well as medical segmentation~\cite{taha2015metrics}. The results from these metrics for the expert as well as averaged novice and practitioners are showcased in Fig.~\ref{fig:consistency}. Note that the expert outperforms the novices and practitioners on all self-consistency metrics. The self-consistency metrics showcases precision of annotators. However, labeling bias may still exist, which is expanded on in the Limitations section~\ref{subsec:limitations}. Additional results and statistics including label category usage, labeling time, confidence metrics, and intra- and inter-annotator agreements are provided in Appendix~\ref{subsec:Statistics}. To ensure label quality, all annotators were compensated with bonus pay based on the self-consistency QA metrics. Also, to ensure novice retention across all $480$ sections, the annotators were paid on a prorated pay, in which the final 160 section annotations are worth increasingly more for every 10 sections annotated. Further details regarding payscales are presented in Appendix~\ref{subsec:MTurk_compensation}. 
\begin{figure}[t]
\centering
\includegraphics[scale =.3]{neurips_data_2023/Figs/consistency.png}
\vspace{-1.5mm}
\caption{Consistency metrics (section-wise) across $120$ repeated sections.}\label{fig:consistency}\vspace{-3mm}
\end{figure}
\paragraph{Annotation Challenges} We present annotations from practitioners, novices, and the expert in Fig.~\ref{fig:challenges}. Fig.~\ref{fig:challenges} showcases (i) the challenges within the dataset, and (ii) expert knowledge that allows overcoming these challenges. The main challenges are diversity, granularity, angular changes, and connected faults. Diversity refers to the wide variety of faults at different locations within the volume. Granularity refers to faults that are harder to distinguish due to a inconsistent shape or blending with surrounding lithographic reflections. Angular changes refers to faults that branch out in multiple directions. Connected faults refer to faults that intersect with each other. Note that the existence of connected faults motivates the need to include both semantic segmentation and instance segmentation tasks. From a semantic segmentation perspective, a connected fault can be viewed as a single entity, but from an instance segmentation perspective, they are separate instances. Additionally, visualizing these challenges, provides insight into the knowledge requirements of experts. For example, by looking at the diversity and granularity columns, we see that the expert is better able to identify faults in diverse regions of the seismic section as well as more difficult to identify faults compared to both the practitioner and novice. Furthermore, the expert is more proficient at capturing complex fault geometries such as angles and connections between faults compared to non-experts. Additionally, there is a qualitative improvement in annotations when going from novices to practitioner labels. This demonstrates the need to understand label disagreement at multiple expertise levels. 


==> Sections/4_Results.tex <==
\section{Experiments}
\label{sec:Experiments}
In this section, we demonstrate the following on the bounding box annotations from Table~\ref{tab:stats_data}:
\begin{itemize}
    \item In Section~\ref{subsec:Model-free}, we provide a sanity check to showcase that the obtained annotations from novices and practitioners are useful for fault delineation.
    \item In Section~\ref{subsec:Detect}, we showcase the value of adding novice and practitioner labels to existing ML workflows for the applications of fault detection and fault instance segmentation.
    \item In Section~\ref{subsec:SSL}, we demonstrate the utility of \texttt{CRACKS} dataset for self-supervised learning under the presence of large, albeit noisy, labels.
    \item Finally, in Section~\ref{subsec:Semantic}, we show that section-wise segmentation using state-of-the-art segmentation models fail on imbalanced \texttt{CRACKS} data.
\end{itemize}

The detailed statistics of the dataset that are used for model training and evaluation is shown in Table \ref{tab:stats_data}. Note that inference is always evaluated against expert labels. The goal is to utilize the available novice and practitioner labels to approximate expert annotations, all on the same seismic images. In this paper, we do not utilize the orange \emph{No Fault (certain)} labels. Also, no differentiation is made between certain and uncertain labels. Both sets of labels are treated as faults. In Appendix~\ref{sec:AppE}, we provide additional results that fuse between certain and uncertain labels. Also, in accordance with fault delineation literature~\cite{dou2021attention, mustafa2024visual} around $10\%$ of the expert ground truth ($815$ faults out of $7636$ from unique seismic images) is used during training. Hence, the goal is to adapt the novice and practitioner labels to the expert label domain. This is because, in practical settings, very large volumes of the earth can be surveyed but annotating them via experts in not feasible. We aim to show that crowdsourcing annotations on these volumes
is a viable strategy to analyze subsurfaces.
\begin{figure}[t]
\centering
\includegraphics[scale =.3]{neurips_data_2023/Figs/pairwise.png}
\vspace{-1.5mm}
\caption{Sanity check to demonstrate that the novice and practitioner annotations are not trivial. Pairwise mIOU between annotations from every practitioner and novice (\texttt{x-axis}) is calculated against the expert annotation and is presented on the \texttt{y-axis}.}\label{fig:model_free}\vspace{-3mm}
\end{figure}


\subsection{Model-free Results}
\label{subsec:Model-free}
Since the same annotations occur across the same seismic sections and faults, we run the mIOU, DICE, and Hausdorff distance metrics between all sections. In Figure \ref{fig:model_free}, we show the distribution of mIOU scores calculated between the annotated seismic sections of each annotator and the expert annotator. We show the distribution of mIOU scores across all sections with an associated box and whisker plot for each annotator. The scores indicate that the novices and practitioners are not producing trivial annotations and each are acting to label an approximation of the true fault distribution of the dataset. Hence, all the novice and practitioner annotations can be considered as noisy labels of the true expert ground truths. Recent works in natural images~\cite{wei2021learning} and medical images~\cite{ju2022improving} tackle this noisy label phenomenon. However, as demonstrated in Fig.~\ref{fig:challenges}, the disagreements among novices and practitioners, and between them, is considerably large. This is because of the knowledge gap between experts and practitioners, and practitioners and novices.

\input{neurips_data_2023/Tables/3_DetectionSegmentation_yolov5}

\subsection{Detection and Instance Segmentation}
\label{subsec:Detect}
Fault detection is the first step of the fault delineation process. For the detection task, we convert the segmentation masks provided by annotators into surrounding bounding boxes. We then train a YOLOv5-l \cite{glenn_jocher_2022_7347926} object detector for each annotator's label set. All models are trained for 100 epochs with an image size of 640 pixels.  For the expert training set, we train with $815$ faults from 40 sections; for novices and practitioners, we use all available faults across 400 sections. We evaluate all models using $6821$ faults from the expert (Table~\ref{tab:stats_data}). Additionally, we fuse the labels from practitioners and novices to create a new training set. Simple classification experiments have benefited from majority voting~\cite{sheng2008get} from MTurk data. In our fusion strategy (rows 6 and 7 in Table~\ref{yolodetectionresults}), we give practitioner labels twice the weight of novice labels. We also perform experiments where expert data is used to fine-tune models previously trained on novice or practitioner data for both the segmentation and detection tasks. We display all results for the expert test set in Table \ref{yolodetectionresults}. 

Next, we perform fault instance segmentation where the goal is to segment specific instances of different faults present in the seismic volume. For the instance segmentation task, we convert the segmentation masks provided by annotators into polygon annotations. We then train a YOLOv5l-seg \cite{glenn_jocher_2022_7347926} instance segmentation model for each annotator's label set. We follow the same procedure as detection for all experiments. We display all results for the expert test set in Table \ref{yolodetectionresults}. For both detection and instance segmentation, we observe that models fine-tuned with expert data show superior performance compared to those trained solely on expert data. This demonstrates that incorporating labels from both practitioners and novices significantly enhances model performance for fault detection compared to using exclusively the expert's training data.

\begin{figure}[t]
\centering
\includegraphics[scale =.3]{neurips_data_2023/Figs/seg_training.png}
\vspace{-1.5mm}
\caption{SSL finetuning on each annotator subset.}\label{fig:ssl}\vspace{-3mm}
\end{figure}

\subsection{Self-supervised Experiments}
\label{subsec:SSL}
In Figure \ref{fig:ssl}, we demonstrate the potential of \texttt{CRACKS} to serve as a new type of benchmark within the context of self supervised learning. To do this, we take the original fault labeled dataset on the semantic segmentation task for each annotator and extract out the cropped region where the annotation occurs. This forms a dataset consisting of object crops where each crop represents where the annotator believes a fault exists. We train a ResNet18 \cite{he2016deep} with the SimCLR \cite{chen2020simple} contrastive learning algorithm for 100 epochs on the overall pool of fault region crops. The training uses a stochastic gradient optimizer (SGD), .001 learning rate, and the default augmentation policy as the original paper. Next, we attach a segmentation head from the UNet \cite{ronneberger2015u} architecture and freeze the weights of the backbone ResNet18 network. We then fine-tune the segmentation head on each individual annotator labeled object crop dataset for 50 epochs with a binary cross-entropy loss, SGD optimizer, and a learning rate of .001. Each model is tested on the same held out expert testing fault object crop segmentation data. The distribution of the IOU scores for each annotator on the expert test set are visually shown as a box and whisper plot in Figure \ref{fig:ssl}. We highlight all annotators in green where the median of the box and whisper plot of their IOU scores is above the overall average of model free comparisons with the expert from Figure \ref{fig:model_free}. We note that leveraging SSL algorithms can noticeably improve fault segmentation performance despite the difficulty of the associated task. 

\input{neurips_data_2023/Tables/4_SOTASegmentation}

%\input{neurips_data_2023/Tables/SOTAsegAfterfine}

\subsection{Section-wise Segmentation}
\label{subsec:Semantic}
For the segmentation task, we evaluate the dataset using State-Of-The-Art (SOTA) segmentation models that includes SegFormer \cite{xie2021segformer}, UNet \cite{ronneberger2015u}, UNet++ \cite{zhou2018unet++}, and DeepLab v3 \cite{chen2017rethinking} (ResNet-50 \cite{he2016deep} as the backbone). Training choices include the cross-entropy loss, Adam optimizer \cite{kingma2017adam}, and 100 epochs of training. We also consider two types of training settings: novice training on top of the pre-trained SOTA network and fine-tuning these trained models with additional expert data. We refer to these settings as before and after fine-tuning respectively. These results are shown in Table \ref{table:segmentation_results_beforefine}. We note poor performance scores across all SOTA models. Additionally, further expert fine-tuning worsens Hausdorff distance metric or causes statistically insignificant changes. This, along with the results of Figure \ref{fig:ssl} showcases the difficulty of the fault segmentation task, which motivates further advancements in segmentation training paradigms to address the challenges of this dataset as discussed previously in Figure \ref{fig:challenges}. Additional results are presented in Appendix~\ref{sec:AppE}.



%\input{neurips_data_2023/Tables/instance_segmentation_yolov5}


==> Sections/5_Discussion.tex <==
\section{Discussion and Conclusion}

\subsection{Limitations}
\label{subsec:limitations}
\paragraph{Labeling bias} Geophysicists who label faults in seismic sections generally do so based on applications they are interested in. For instance, geophysicists monitoring earthquakes are only interested in active faults that cause rocks to move laterally. Geophysicists looking for carbon sequestration are only interested in sealing faults that do not allow movements between rocks. Hence, datasets constructed on seismic sections of interest might have differently labeled faults based on the geophysicist labeling it~\cite{mustafa2024visual}. In practice, the time-consuming nature of segmenting each fault as well as the vast quantity of subsurface data in the earth, precludes having multiple experts looking at the same faults. In this paper, we provide consistency of labeling the same frames across time as quality control to ensure that the expert is precise. However, bias may exist, depending on specific task requirements.

\paragraph{2D vs 3D labeling} In this paper, we choose to annotate faults on 2D sections, even though the F3 dataset is available in 3D. We do so because of two reasons. Firstly, it is not trivial to extend MTurk software to work on 3D data. Existing methods that annotate 3D images treat them as 2D data which are postprocessed~\cite{giuly2013dp2}. This is an additional workflow, which is not the aim of the paper. Moreover, evaluation of 3D segmented faults is done in 2D~\cite{li2022automatic}. However, the $400$ annotated sections in our dataset are contiguous frames that make up the volume and further methods can be developed that treat fault annotations as 3D data.

\paragraph{Visual labeling only} During the annotation process, the expert was instructed to only utilize visual seismic data and work on MTurk software, to not bias the expert labels against the novices and practitioners. However, in practice, geophysicists utilize specialized software like OpendTect~\cite{dgbpy_2019} and use multi-modal data including well logs, rock properties, and elastic impedance among others to segment difficult faults. In this paper, we have specifically chosen F3 subsurface data to annotate faults since the faults in the Netherlands North Sea are easier to visually inspect and label.

\subsection{Conclusion} 
The \texttt{CRACKS} dataset presents the first subsurface fault-labeled data on the F3 seismic volume using resources from crowdsourcing platforms. \texttt{CRACKS} allows the study of annotation disagreement within and between expertise levels on the non-common knowledge task of seismic fault delineation. The experimental design provides real-world case studies where the underlying images in the train and test sets are the same. However, the labels in the crowdsourced data can be considered as noisy versions of the true ground truth labels, thereby significantly challenging existing ML paradigms. This is a common occurrence in medical data and even more in seismic images where the vast regions in the earth's subsurface are not surveyed and hence, the physical properties unknown. \texttt{CRACKS} provides the first foray into analyzing and delineating subsurface faults based on novices from crowdsourcing platforms.

==> Tables/1_Stats.tex <==
\begin{table}[t]
\begin{center}
\begin{sc}
\begin{tiny}
\caption{Statistics of the available data modalities in the train and test sets.}
\begin{tabular}{lllllllll}
\toprule
\multicolumn{1}{c}{\multirow{3}{*}{Expertise}} & \multicolumn{4}{c}{Train Total} & \multicolumn{4}{c}{Test Total} \\ %$& \multicolumn{1}{c}{\multirow{2}{*}{Crowdsourcing statistics}} \\
\multicolumn{1}{c}{}                           & \multicolumn{2}{c}{Bounding boxes}       & \multicolumn{2}{c}{percentage of pixels(\%)}      & \multicolumn{2}{c}{Bounding boxes}      & \multicolumn{2}{c}{percentage of pixels(\%)}                                                \\ \cline{2-5} \cline{6-9}
\multicolumn{1}{c}{}                           & {Certain}       & {Uncertain}      &  {Certain}      & {Uncertain}      & {Certain}       & {Uncertain}      &  {Certain}      & {Uncertain} \\ \midrule
Geophysicist                                   &       118       &        697          &        0.4844     &        2.0554            & 732     & 6089            & 0.3416     & 2.1265  \\
Practitioners                                  &              11376 &         36688     &              0.6480 &         1.6992       &       ---      &       ---        &       ---      &       --- \\
Novices                                        &      84650        &       91379           &      1.6762        &       1.9238           &     ---        &     ---          &     ---        &     ---     \\ \bottomrule
\end{tabular}
\label{tab:stats_data}
\end{tiny}
\end{sc}
\end{center}
\end{table}



==> Tables/2_DatasetCompare.tex <==
\begin{table}[t]
\begin{center}
\begin{tiny}
\begin{sc}
\caption{Comparison of datasets containing multiple annotations per sample and multiple levels of expertise in annotations.}
\begin{tabular}
{p{0.12\textwidth}p{0.12\textwidth}p{0.12\textwidth}p{0.1\textwidth}p{0.1\textwidth}p{0.08\textwidth}p{0.04\textwidth}p{0.04\textwidth}p{0.15\textwidth}}
\toprule
\textbf{Dataset} & \textbf{Expertise} & \textbf{Annotations per Sample} & \textbf{Annotation Confidence} & \textbf{Resolution} & \textbf{Samples} & \textbf{Classes} &  \textbf{Total Annotations} \\ 
\toprule
CIFAR10-H \cite{peterson2019human}       & Novices (2,571)       &  50    &   \ding{55}   &       32x32       &       10,000       &       10       &       500k       \\ 
CIFAR-10S \cite{collins2022eliciting}       & Novices (248)              &       6       &       \ding{51} (3)     &       32x32       &       1,000       &       10       &       6,200       \\ 
\midrule
LIDC-IDRI \cite{armato2011lung}       & Experts (12 radiologists)       &       4       &       \ding{55}       &       512x512       &       1018       &       2       &       4,072       \\ 
MICCAI2012 \cite{litjens2012pattern}       & Experts (observers)                          &            3                               &          \ding{55}                  &              320x320               &  48 &  2 & 144\\ 
RIGA \cite{almazroa2017agreement}       & Experts (6 ophthalmologists)       &       6       &    \ding{55}                        &           2160x1440       &  750          &  2 & 4500\\ 
QUBIQ \cite{menzequantification}       & Experts&       4       &       \ding{55}       &       N/A (>640x640)       &       268       &       3       &       1049       \\ \midrule
Phrase Detectives Corpus V2 \cite{poesio2019crowdsourced}       &  Novices (1958), Experts (2)       &       20       &       \ding{55}       &       N/A       &       108,000       &       3       &       2.2M       \\ \midrule
         % &                       &                                         &                            &                            &  &  \\ \hline
\texttt{CRACKS}         & Novices (26), practitioners (8), expert (1)                     & 35                                        &    \ding{51}  (3)                       &       701x255                     &  7636  & 3 &  231729  \\ \bottomrule
\end{tabular}
\label{tab:stats_datasets}
\end{sc}
\end{tiny}
\end{center}
\end{table}

==> Tables/3_DetectionSegmentation_yolov5.tex <==
\begin{table}[t]
\begin{center}
\begin{tiny}
\begin{sc}
\caption{Results of fault detection and instance segmentation for different training sets and methods using mean Average Precision at 0.5. The best results in each application are bolded.}
\begin{tabular}{lcr}
\toprule
Training Set  & \multicolumn{1}{c}{Detection} & Instance Segmentation  \\
\midrule

Expert     & 0.425 ± 0.004   &      0.145 ± 0.002      \\
\midrule
Novice (Average)     & 0.219 ± 0.001   &  0.051 ± 0.001            \\
Practitioner (Average)     & 0.278 ± 0.001     &  0.074 ± 0.001       \\
\midrule
Novice expert fine-tuned (Average)     & 0.460 ± 0.001   &    0.146 ± 0.001        \\
Practitioner expert fine-tuned (Average)      & \textbf{0.466 ± 0.001}  &  0.152 ± 0.001            \\ 
\midrule
Practitioner+Novice (Label Fusion)     & 0.354 ± 0.004      &   0.103 ± 0.002      \\
Practitioner+Novice (Label Fusion) expert fine-tuned      & 0.457 ± 0.003      &  \textbf{0.177 ± 0.002}         \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\label{yolodetectionresults}
\end{sc}
\end{tiny}
\end{center}
\end{table}

==> Tables/4_SOTASegmentation.tex <==
\begin{table}[h!]
\begin{center}
\begin{scriptsize}
\begin{sc}
\caption{Averaged novice and practitioner Section-wise Fault Segmentation Results before and after finetuning on expert. Hausdorff distance shows significant decrease (in red) while all other changes are statistically insignificant.}
\begin{tabular}{lcccccr}
\toprule
Models & \multicolumn{3}{c}{Before Finetuning} & \multicolumn{3}{c}{After finetuning}\\ 
& mIOU & Hausdorff & DICE Score & mIOU & Hausdorff & DICE Score \\
\midrule
Segformer \cite{xie2021segformer}                          & 0.53  & 41.7  & 0.58 & 0.54 & \color{red}{59.1} & 0.56  \\
Unet \cite{ronneberger2015u}                            & 0.48  & 74.5  & 0.49 & 0.48 & \color{red}{87.6} & 0.5  \\
Unet++ \cite{zhou2019unetplusplus}                     & 0.49  & 75.53 & 0.5 & 0.49 & \color{red}{98.9} & 0.51  \\
Deeplab v3 (Resenet 50 \cite{he2016deep}) \cite{chen2017deeplab}   & 0.48  & 54.7  & 0.53 & 0.48 & \color{red}{122.1} & 0.51 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\label{table:segmentation_results_beforefine}
\end{sc}
\end{scriptsize}
\end{center}
\end{table}

==> Tables/Archived_instance_segmentation_yolov5.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}cc@{}}
\toprule
\multicolumn{1}{c}{ Fault Instance Segmentation Results with YOLOv5}   
\\ \midrule
\multicolumn{1}{c}{Training Set}  & \multicolumn{1}{c}{Mask mAP0.5} \\
\midrule

Expert (40 Images)    & 0.145               \\
Novice (Average)     & 0.051              \\
Practitioner (Average)     & 0.074               \\
Novice fine-tuned with  Expert (Average)    & 0.146               \\
Practitioner fine-tuned with Expert (Average)    & 0.152               \\
Practitioner+Novice (Label Fusion)     & 0.103               \\
Practitioner+Novice (Label Fusion)  fine-tuned with  Expert      & \textbf{0.177}               \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{  Results of instance segmentation for different training sets}
\label{yolosegmentationresults}
\end{table}

==> Tables/DetectionmodelsALL.tex <==
\begin{table}[t]
\begin{center}
\begin{tiny}
\begin{sc}
\caption{Results of fault detection for different training sets and methods using mean Average Precision at 0.5.}
\begin{tabular}{lcccc}
\toprule
Training Set & YOLO v5 & Faster R-CNN & RetinaNet \\
\midrule
Expert & 0.425 & 0.392 & 0.321 \\
\midrule
Novice (Average) & 0.219 & 0.177 & 0.129 \\
Practitioner (Average) & 0.278 & 0.213 & 0.213 \\
\midrule
Novice expert fine-tuned (Average) & 0.460 & 0.401 & 0.386 \\
Practitioner expert fine-tuned (Average) & {0.466} & 0.420 & 0.386 \\
\midrule
Practitioner+Novice (Label Fusion) & 0.354 & 0.331 & 0.248 \\
Practitioner+Novice (Label Fusion) expert fine-tuned & 0.441 & {0.425} & 0.384 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\label{yolodetectionresults}
\end{sc}
\end{tiny}
\end{center}
\end{table}



==> Tables/DomainSpecific.tex <==
\begin{table}[h!]
\begin{center}
\begin{tiny}
\begin{sc}
\caption{Section-wise fault segmentation results for domain specific models compared against SimCLR. The results are averaged across all novices and practitioners.}
\setlength{\tabcolsep}{4.3pt}
\begin{tabular}{lccccccccr}
\toprule
Models & \multicolumn{3}{c}{Novices} & \multicolumn{3}{c}{Practitioners} & \multicolumn{3}{c}{Expert}\\ 
& mIOU & DICE & Hauss. & mIOU & DICE & Hauss. & mIOU & DICE & Hauss. \\
\midrule
SimCLR & $.6 \pm .05$ & $.73 \pm .04$ & $13.72 \pm .73$ & $.61 \pm .05$ & $.74 \pm .05$ & $13.36 \pm .8$ & $.64$ & $.77$ & $12.85$ \\
\midrule
Volumetric & \textbf{$.6 \pm .03$} & \textbf{$.74 \pm .03$} & $13.52 \pm .98$ & $.6 \pm .06$ & $.73 \pm .06$ & $13.87 \pm .99$ & $.65$ & $.78$ & $12.6$ \\
FaultSeg3D & $.005 \pm .002$ & $.04 \pm .015$ & $281 \pm 36.58$ & $.005 \pm .001$ & $.04 \pm .009$ & $273.16 \pm 16.8$ & $.006$ & $.06$ & $397.97$ \\
FaultNet & $.023 \pm .01$ & $.09 \pm .03$ & $226.62 \pm 88.3$ & $.024 \pm .007$ & $.097 \pm .021$ & $224 \pm 33.1$ & $.05$ & $.14$ & $195.2$ \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\label{table:segmentation_results_sub}
\end{sc}
\end{tiny}
\end{center}
\end{table}



==> Tables/LabelFusion_Certain.tex <==
\begin{table}[t]
\begin{center}
\begin{tiny}
\begin{sc}
\caption{Results of fault detection and instance segmentation for label fusion between certain and uncertain labels using mean Average Precision at 0.5. }
\begin{tabular}{lcr}
\toprule
Training Set  & \multicolumn{1}{c}{Detection} & Instance Segmentation  \\
\midrule

Certain-Uncertain Label Fusion     & 0.308 ± 0.004   &      0.458 ± 0.002      \\

Certain-Uncertain Label Fusion (expert fine-tuned)    & 0.425 ± 0.004   &      0.168 ± 0.002      \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\label{table:labelfusioncertain}
\end{sc}
\end{tiny}
\end{center}
\end{table}

==> Tables/LabelFusion_alphaexpertise.tex <==
\begin{table}[t]
\begin{center}
\begin{tiny}
\begin{sc}
\caption{Results of fault detection and instance segmentation for label fusion between practitioner and novices with different alpha parameters $(\alpha \times Novice + (1-\alpha) \times Practitioner) $ using mean Average Precision at 0.5.  }
\begin{tabular}{lcr}
\toprule
Training Set Label Fusion Alpha Parameter   & \multicolumn{1}{c}{Detection} & Instance Segmentation  \\
\midrule


Label Fusion $\alpha=0$     & 0.342  &    0.118     \\
Label Fusion $\alpha=0.2$     & 0.329  &    0.0535     \\
Label Fusion $\alpha=0.4$     & 0.325  &   0.0433      \\
Label Fusion $\alpha=0.5$     & 0.328  &     0.0813    \\
Label Fusion $\alpha=0.6$     & 0.336  &    0.0892     \\
Label Fusion $\alpha=0.8$     & 0.324  &   0.00249      \\
Label Fusion $\alpha=1$     & 0.317  &    0.0808     \\
\midrule
Label Fusion $\alpha=0$  (expert fine-tuned)     &  0.457 &  0.16     \\
Label Fusion $\alpha=0.2$  (expert fine-tuned)    & 0.465  &   0.154  \\
Label Fusion $\alpha=0.4$  (expert fine-tuned)    & 0.458  &    0.145     \\
Label Fusion $\alpha=0.5$  (expert fine-tuned)    & 0.465  &  0.168       \\
Label Fusion $\alpha=0.6$  (expert fine-tuned)     & 0.445  &      0.149   \\
Label Fusion $\alpha=0.8$  (expert fine-tuned)    & 0.449  &     0.134    \\
Label Fusion $\alpha=1$  (expert fine-tuned)    & 0.438  &     0.143    \\

\bottomrule
\end{tabular}
\vspace*{.1mm}
\label{table:labelfusionalpha}
\end{sc}
\end{tiny}
\end{center}
\end{table}

==> Tables/SOTAsegAfterfine.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{4}{c}{Fault Semantic Segmentation Results with SOTA models fintuned on expert labels} \\ \midrule
\multicolumn{1}{c}{Models} & \multicolumn{1}{c}{mIoU} & \multicolumn{1}{c}{Hausdorff distance} & \multicolumn{1}{c}{Dice score} \\ \midrule
Segformer                          & 0.54  & 59.1  & 0.56  \\
Unet                            & 0.48  & 87.6  & 0.5  \\
Unet++                      & 0.49  & 98.9 & 0.51  \\
Deeplab v3 (Resenet 50)     & 0.48  & 122.1  & 0.51  \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Results of fault instance segmentation using different training sets}
\label{table:segmentation_results_afterfine}

\end{table}

==> Tables/SOTAsegmentation_sup.tex <==
\begin{table}[h!]
\begin{center}
\begin{scriptsize}
\begin{sc}
\caption{Averaged novice and practitioner Section-wise Fault Segmentation Results before and after finetuning on expert. Hausdorff distance shows significant decrease (in red) while all other changes are statistically insignificant. These are the results of training the models multiple times using different seeds.}
\begin{tabular}{lcccccr}
\toprule
Models & \multicolumn{3}{c}{Before Finetuning} & \multicolumn{3}{c}{After finetuning}\\ 
& mIOU & Hausdorff & DICE Score & mIOU & Hausdorff & DICE Score \\
\midrule
Segformer \cite{xie2021segformer}                          & 0.53 ± 0.003  & 42.4 ± 0.6 & 0.58 ± 0.0005 & 0.54 ± 0.002 & \color{red}{59.57 ± 0.52} & 0.56 ± 0.004  \\
Unet \cite{ronneberger2015u}                            & 0.49 ± 0.006  & 69.09 ± 4.68  & 0.5 ± 0.02 & 0.49 ± 0.006 & \color{red}{90.36 ± 1.66} & 0.5 ± 0.007  \\
Unet++ \cite{zhou2019unetplusplus}                     & 0.49 ± 0.004  & 69.44 ± 5.27  & 0.51 ± 0.009 & 0.49 ± 0.0012  & \color{red}{92.8 ± 5.28} & 0.51 ± 0.001  \\
Deeplab v3 \cite{chen2017deeplab}   & 0.48 ± 0.002  & 56.8 ± 2.13  & 0.52 ± 0.002 & 0.48 ± 0.0002 & \color{red}{123.9 ± 1.57} & 0.517 ± 0.0003  \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\label{table:segmentation_results_sub}
\end{sc}
\end{scriptsize}
\end{center}
\end{table}

==> Tables/faultdatasets.tex <==
\begin{table}[t]
\begin{center}
\scriptsize
{
\caption{Summary of various seismic datasets and their characteristics.}
\begin{tabular}{p{2.5cm}p{1cm}p{1cm}p{3cm}p{1.5cm}p{1.5cm}}
Dataset          & Type    & Dim. & Size                               & Multi-source labeling & Fault labels \\
\hline
LANDMASS 1       & Seismic & 2D   & 17667 batches of 99x99             & No                    & Y            \\
LANDMASS 2       & Seismic & 2D   & 4000 batches of 150x300            & No                    & Y            \\
F3 (SFD-CNN-TL)  & Seismic & 2D   & 503 patches of 45x45               & No                    & Y            \\
Great South Basin (GSB) & Seismic & 3D   & Covers 1345 km with 12.5m spacing & No                    & Y            \\
Thebe            & Seismic & 3D   & 1803x3174x1537                     & No                    & Y            \\
Opunake-3D       & Seismic & 3D   & Covers area 215 km                 & No                    & N            \\
GN1101           & Seismic & 3D   & 442.25 km with 12.5m x 25m spacing & No                    & Private      \\
FaultSeg3D       & Synthetic & 3D & 128x128x128                        & No                    & Y            \\
\textbf{CRACKS}           & \textbf{Seismic} & \textbf{3D}   &        \textbf{800x701x255}          & \textbf{Yes}                   & \textbf{Yes}          
\end{tabular}
}
\end{center}

\label{table:seismic_datasets}
\end{table}

==> neurips_data_2023/Tables/Archived_instance_segmentation_yolov5.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}cc@{}}
\toprule
\multicolumn{1}{c}{ Fault Instance Segmentation Results with YOLOv5}   
\\ \midrule
\multicolumn{1}{c}{Training Set}  & \multicolumn{1}{c}{Mask mAP0.5} \\
\midrule

Expert (40 Images)    & 0.145               \\
Novice (Average)     & 0.051              \\
Practitioner (Average)     & 0.074               \\
Novice fine-tuned with  Expert (Average)    & 0.146               \\
Practitioner fine-tuned with Expert (Average)    & 0.152               \\
Practitioner+Novice (Label Fusion)     & 0.103               \\
Practitioner+Novice (Label Fusion)  fine-tuned with  Expert      & \textbf{0.177}               \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{  Results of instance segmentation for different training sets}
\label{yolosegmentationresults}
\end{table}

==> neurips_data_2023/Tables/DetectionmodelsALL.tex <==
\begin{table}[t]
\begin{center}
\begin{tiny}
\begin{sc}
\caption{Results of fault detection for different training sets and methods using mean Average Precision at 0.5.}
\begin{tabular}{lcccc}
\toprule
Training Set & YOLO v5 & Faster R-CNN & RetinaNet \\
\midrule
Expert & 0.425 & 0.392 & 0.321 \\
\midrule
Novice (Average) & 0.219 & 0.177 & 0.129 \\
Practitioner (Average) & 0.278 & 0.213 & 0.213 \\
\midrule
Novice expert fine-tuned (Average) & 0.460 & 0.401 & 0.386 \\
Practitioner expert fine-tuned (Average) & {0.466} & 0.420 & 0.386 \\
\midrule
Practitioner+Novice (Label Fusion) & 0.354 & 0.331 & 0.248 \\
Practitioner+Novice (Label Fusion) expert fine-tuned & 0.441 & {0.425} & 0.384 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\label{yolodetectionresults}
\end{sc}
\end{tiny}
\end{center}
\end{table}



==> neurips_data_2023/Tables/DomainSpecific.tex <==
\begin{table}[h!]
\begin{center}
\begin{tiny}
\begin{sc}
\caption{Section-wise fault segmentation results for domain specific models compared against SimCLR. The results are averaged across all novices and practitioners.}
\setlength{\tabcolsep}{4.3pt}
\begin{tabular}{lccccccccr}
\toprule
Models & \multicolumn{3}{c}{Novices} & \multicolumn{3}{c}{Practitioners} & \multicolumn{3}{c}{Expert}\\ 
& mIOU & DICE & Hauss. & mIOU & DICE & Hauss. & mIOU & DICE & Hauss. \\
\midrule
SimCLR & $.6 \pm .05$ & $.73 \pm .04$ & $13.72 \pm .73$ & $.61 \pm .05$ & $.74 \pm .05$ & $13.36 \pm .8$ & $.64$ & $.77$ & $12.85$ \\
\midrule
Volumetric & \textbf{$.6 \pm .03$} & \textbf{$.74 \pm .03$} & $13.52 \pm .98$ & $.6 \pm .06$ & $.73 \pm .06$ & $13.87 \pm .99$ & $.65$ & $.78$ & $12.6$ \\
FaultSeg3D & $.005 \pm .002$ & $.04 \pm .015$ & $281 \pm 36.58$ & $.005 \pm .001$ & $.04 \pm .009$ & $273.16 \pm 16.8$ & $.006$ & $.06$ & $397.97$ \\
FaultNet & $.023 \pm .01$ & $.09 \pm .03$ & $226.62 \pm 88.3$ & $.024 \pm .007$ & $.097 \pm .021$ & $224 \pm 33.1$ & $.05$ & $.14$ & $195.2$ \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\label{table:segmentation_results_sub}
\end{sc}
\end{tiny}
\end{center}
\end{table}



==> neurips_data_2023/Tables/SOTAsegAfterfine.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{4}{c}{Fault Semantic Segmentation Results with SOTA models fintuned on expert labels} \\ \midrule
\multicolumn{1}{c}{Models} & \multicolumn{1}{c}{mIoU} & \multicolumn{1}{c}{Hausdorff distance} & \multicolumn{1}{c}{Dice score} \\ \midrule
Segformer                          & 0.54  & 59.1  & 0.56  \\
Unet                            & 0.48  & 87.6  & 0.5  \\
Unet++                      & 0.49  & 98.9 & 0.51  \\
Deeplab v3 (Resenet 50)     & 0.48  & 122.1  & 0.51  \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Results of fault instance segmentation using different training sets}
\label{table:segmentation_results_afterfine}

\end{table}

==> neurips_data_2023/Tables/faultdatasets.tex <==
\begin{table}[t]
\begin{center}
\scriptsize
{
\caption{Summary of various seismic datasets and their characteristics.}
\begin{tabular}{p{2.5cm}p{1cm}p{1cm}p{3cm}p{1.5cm}p{1.5cm}}
Dataset          & Type    & Dim. & Size                               & Multi-source labeling & Fault labels \\
\hline
LANDMASS 1       & Seismic & 2D   & 17667 batches of 99x99             & No                    & Y            \\
LANDMASS 2       & Seismic & 2D   & 4000 batches of 150x300            & No                    & Y            \\
F3 (SFD-CNN-TL)  & Seismic & 2D   & 503 patches of 45x45               & No                    & Y            \\
Great South Basin (GSB) & Seismic & 3D   & Covers 1345 km with 12.5m spacing & No                    & Y            \\
Thebe            & Seismic & 3D   & 1803x3174x1537                     & No                    & Y            \\
Opunake-3D       & Seismic & 3D   & Covers area 215 km                 & No                    & N            \\
GN1101           & Seismic & 3D   & 442.25 km with 12.5m x 25m spacing & No                    & Private      \\
FaultSeg3D       & Synthetic & 3D & 128x128x128                        & No                    & Y            \\
\textbf{CRACKS}           & \textbf{Seismic} & \textbf{3D}   &        \textbf{800x701x255}          & \textbf{Yes}                   & \textbf{Yes}          
\end{tabular}
}
\end{center}

\label{table:seismic_datasets}
\end{table}
